Spring Embedders and Force Directed Graph Drawing Algorithms

Force-directed algorithms are among the most flexible methods for calculating layouts of simple undirected graphs. Also known as spring embedders, such algorithms calculate the layout of a graph using only information contained within the structure of the graph itself, rather than relying on domain-specific knowledge. Graphs drawn with these algorithms tend to be aesthetically pleasing, exhibit symmetries, and tend to produce crossing-free layouts for planar graphs. In this survey we consider several classical algorithms, starting from Tutte's 1963 barycentric method, and including recent scalable multiscale methods for large and dynamic graphs.

==> Makefile <==
TEX_FILE=fd_survey

paper:
	latex $(TEX_FILE).tex
	bibtex $(TEX_FILE)
	latex $(TEX_FILE).tex
	latex $(TEX_FILE).tex

	dvips -Ppdf -G0 -o $(TEX_FILE).ps $(TEX_FILE).dvi

	ps2pdf -sPAPERSIZE=letter \
	-dMaxSubsetPct=100 -dCompatibilityLevel=1.3 \
	-dSubsetFonts=true -dEmbedAllFonts=true \
	-dAutoFilterColorImages=false \
	-dAutoFilterGrayImages=false \
	-dColorImageFilter=/FlateEncode \
	-dGrayImageFilter=/FlateEncode \
	-dModoImageFilter=/FlateEncode \
	$(TEX_FILE).ps $(TEX_FILE).pdf


